Sphynx: ReLU-Efficient Network Design for Private Inference

The emergence of deep learning has been accompanied by privacy concerns surrounding users' data and service providers' models. We focus on private inference (PI), where the goal is to perform inference on a user's data sample using a service provider's model. Existing PI methods for deep networks enable cryptographically secure inference with little drop in functionality; however, they incur severe latency costs, primarily caused by non-linear network operations (such as ReLUs). This paper presents Sphynx, a ReLU-efficient network design method based on micro-search strategies for convolutional cell design. Sphynx achieves Pareto dominance over all existing private inference methods on CIFAR-100. We also design large-scale networks that support cryptographically private inference on Tiny-ImageNet and ImageNet.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{sec: introduction} and abstract.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec: related works}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section~\ref{subsec: experimental setup} and Appendix~\ref{appendix: hyperparameters protocols}. Code included in a zip file with supplementary materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{subsec: experimental setup} and Appendix~\ref{appendix: hyperparameters protocols}. }
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Figure~\ref{fig: reduce loc search vs default}, Table~\ref{table: cifar100}, Figure~\ref{fig: ablations studies}, and Table~\ref{table: vanilla vs separable details}. We performed multiple random seed experiments related to CIFAR-100. Also we conduct ablation studies with multiple random seeds if the performance difference is not significantly large.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{subsec: experimental setup}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{subsec: experimental setup}. We cite the dataset we used in our experiments}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> diagram2.tex <==
%\resizebox{\linewidth}{!}{%neurips
\resizebox{0.9\linewidth}{!}{
\begin{tikzpicture}[font=\sffamily]
    \fontfamily{cmss}
    \tikzstyle{every node}=[font=\scriptsize]
    \node (oneShot) [oneShotModel] {\tiny ReLU Efficient Search Space};
    
    \path (oneShot)+(2.3, 1.5) node (sample) [sampleNode] {\tiny Run Existing NAS Algorithm};
    \path (oneShot)+(4, 0) node (CS) [CSNode] {Find optimized reduce cell location via Gumbel-Softmax Trick};
    \path (oneShot)+(2.3, -1.6) node (restriction) [restrictionNode] {\tiny Restrict $f$ with \emph{minimizer} of $g$};
    
    \path [draw, ->, line width = 0.2mm] (oneShot.north) to (0, 1.5) to (sample.west); 
    \path [draw, ->, line width = 0.2mm] (sample.east) to (4, 1.5) to (CS.north);
    \path [draw, ->, line width = 0.2mm] (CS.south) to (4, -1.6) to (restriction.east);
    \path [draw, ->, line width = 0.2mm] (restriction.north) to (sample.south);
    \backgroundc{oneShot}{oneShot}{oneShot}{oneShot}{orange}{Stage 1};
    \backgroundd{sample}{sample}{CS}{restriction}{green}{Stage 2};

\end{tikzpicture}
}

==> tikz/normal_cell.tex <==
\tikzstyle{Cell}=[draw, fill=gray!10, text width=4.0em, thick, rounded corners=0.3cm,
    text centered, minimum width=4.0em, minimum height=3.0em]
\tikzstyle{SubCell} = [draw, fill=white!10, text width=2.2em, thick, rounded corners=0.2cm,
    text centered, minimum width=3em, minimum height=2.0em]
\tikzstyle{Cell2}=[draw, fill=gray!10, text width=5.0em, thick, rounded corners=0.2cm,
    align=right, minimum width=6.0em, minimum height=3.0em]
\tikzstyle{texto} = [above, text width=20em, text centered]
\tikzstyle{Image}=[draw, fill=gray!10, text width=3.0em, 
    text centered, minimum width=7.0em, minimum height=4.0em
\tikzstyle{Cell3} = [draw, fill=gray!10, text width=5.0em, thick, rounded corners=0.2cm,
    text centered, minimum width=4.0em, minimum height=3.0em]

\tikzstyle{customNode}=[draw, fill=purple!25, text width=1.0em, 
    text centered, minimum width=1.0em, minimum height=1.0em, rounded corners]
\tikzstyle{customNode2}=[draw, fill=green!25, text width=1.0em, 
    text centered, minimum width=1.0em, minimum height=1.0em, rounded corners]
\tikzstyle{operation}=[draw, fill=white!20, text width=2.0em, 
    text centered, minimum width=2.0em, minimum height=1.0em, rounded corners]
    
\resizebox{0.9\linewidth}{!}{
\begin{tikzpicture}[font=\sffamily, trim left={(0.05,0)}, trim right={(2.8,0)}]
    \fontfamily{cmss}
    \tikzstyle{every node}=[font=\scriptsize]
    
    \node (node0) [customNode] {N0};
    \path (node0)+(0.8, 0.6) node (node1) [customNode] {N1};
    \path (node0)+(1.6, 0) node (node2) [customNode] {N2};
    \path (node2)+(1.2, 0) node (node3) [customNode2] {N3};
    
    \path [draw=red!80, ->, >=stealth, line width=0.18em] (node0.north) to [out=90, in=180] (node1.west);
    \path [draw=blue, ->, >=stealth, line width=0.18em] (node1.east) to [out=0, in=90] (node2.north);
    \path [draw=orange, ->, >=stealth, line width=0.18em] (node0.east) to [out=0, in=180] (node2.west);
    \path [draw=black, ->, >=stealth, line width=0.18em] (node2.east) to [out=0, in=180] (node3.west);
    \path [draw=black, ->, >=stealth, line width=0.18em] (node0.south) to [out=320, in=180] (1.4, -0.6) to [out=0, in=220] (node3.south);
    \path [draw=black, ->, >=stealth, line width=0.18em] (node1.east) to [out=0, in=140] (node3.north);
\end{tikzpicture}
}

==> tikz/preproc1.tex <==
%\resizebox{\linewidth}{!}{%neurips
% \usetikzlibrary{quotes,arrows.meta}
\tikzset{
  annotated cuboid/.pic={
    \tikzset{%
      every edge quotes/.append style={midway, auto},
      /cuboid/.cd,
      #1
    }
    \draw [every edge/.append style={pic actions, densely dashed, opacity=.5}, pic actions]
    (0,0,0) coordinate (o) -- ++(-\cubescale*\cubex,0,0) coordinate (a) -- ++(0,-\cubescale*\cubey,0) coordinate (b) edge coordinate [pos=1] (g) ++(0,0,-\cubescale*\cubez)  -- ++(\cubescale*\cubex,0,0) coordinate (c) -- cycle
    (o) -- ++(0,0,-\cubescale*\cubez) coordinate (d) -- ++(0,-\cubescale*\cubey,0) coordinate (e) edge (g) -- (c) -- cycle
    (o) -- (a) -- ++(0,0,-\cubescale*\cubez) coordinate (f) edge (g) -- (d) -- cycle;
    \path [every edge/.append style={pic actions, |-|}]
    (b) +(0,-5pt) coordinate (b1) edge ["$H_i$ \cubeunits"'] (b1 -| c)
    (b) +(-5pt,0) coordinate (b2) edge ["$H_i$ \cubeunits"] (b2 |- a)
    (c) +(3.5pt,-3.5pt) coordinate (c2) edge ["$4C_i$ \cubeunits"'] ([xshift=3.5pt,yshift=-3.5pt]e)
    ;
  },
  /cuboid/.search also={/tikz},
  /cuboid/.cd,
  width/.store in=\cubex,
  height/.store in=\cubey,
  depth/.store in=\cubez,
  units/.store in=\cubeunits,
  scale/.store in=\cubescale,
  width=10,
  height=10,
  depth=10,
  units=cm,
  scale=.1,
}

\tikzset{
  annotated cuboid2/.pic={
    \tikzset{%
      every edge quotes/.append style={midway, auto},
      /cuboid/.cd,
      #1
    }
    \draw [every edge/.append style={pic actions, densely dashed, opacity=.5}, pic actions]
    (0,0,0) coordinate (o) -- ++(-\cubescale*\cubex,0,0) coordinate (a) -- ++(0,-\cubescale*\cubey,0) coordinate (b) edge coordinate [pos=1] (g) ++(0,0,-\cubescale*\cubez)  -- ++(\cubescale*\cubex,0,0) coordinate (c) -- cycle
    (o) -- ++(0,0,-\cubescale*\cubez) coordinate (d) -- ++(0,-\cubescale*\cubey,0) coordinate (e) edge (g) -- (c) -- cycle
    (o) -- (a) -- ++(0,0,-\cubescale*\cubez) coordinate (f) edge (g) -- (d) -- cycle;
    \path [every edge/.append style={pic actions, |-|}]
    % (b) +(0,-5pt) coordinate (b1) edge [" \cubeunits"'] (b1 -| c)
    % (b) +(-5pt,0) coordinate (b2) edge [" \cubeunits"] (b2 |- a)
    (c) +(3.5pt,-3.5pt) coordinate (c2) edge ["$C_i$ \cubeunits"'] ([xshift=3.5pt,yshift=-3.5pt]e)
    ;
  },
  /cuboid/.search also={/tikz},
  /cuboid/.cd,
  width/.store in=\cubex,
  height/.store in=\cubey,
  depth/.store in=\cubez,
  units/.store in=\cubeunits,
  scale/.store in=\cubescale,
  width=10,
  height=10,
  depth=10,
  units=cm,
  scale=.1,
}

\tikzstyle{Phase}=[draw, fill=orange!50, text width=2.0em, thick, rotate=90,
    text centered, minimum width=6.0em, minimum height=2.0em, scale=0.6]
\tikzstyle{Phase2}=[draw, fill=green!50, text width=5.0em, thick, rotate=90,
    text centered, minimum width=6.0em, minimum height=2.0em, scale=0.6]
\tikzstyle{Phase3}=[draw, fill=blue!40, text width=5.0em, thick, rotate=90,
    text centered, minimum width=6.0em, minimum height=2.0em, scale=0.6]
\tikzstyle{texto} = [above, text width=20em, text centered]
\tikzstyle{Cell}=[draw, fill=gray!10, text width=6.0em, thick, 
    text centered, minimum width=6.0em, minimum height=3.0em]
    
\newcommand{\preproc}[6]{%
  \begin{pgfonlayer}{background}
    % Left-top corner of the background rectangle
    \path (#1.north |- #2.east)+(-0.3, 0.5) node (a1) {};
    % Right-bottom corner of the background rectanle
    \path (#3.south |- #4.west)+(+0.3,-0.5) node (a2) {};
    % Draw the background
    \path[fill=#5!10,rounded corners, draw=black!50, dashed]
      (a1) rectangle (a2);
    \path (a1.north |- a1.east)+(1.2, -0.34) node (u1)[texto]
      {\tiny #6};
  \end{pgfonlayer}}

\resizebox{1.0\linewidth}{!}{
\begin{tikzpicture}
%   \pic {annotated cuboid};
%   \pic [fill=magenta, text=blue, draw=blue] at (5,0) {annotated cuboid={width=30, height=5, depth=10}};
%   \pic [fill=green, text=green!50!black, draw=green!25!black] at (5,-2) {annotated cuboid={width=6, height=20, depth=15, units=mm}};
%   \pic at (1,-3) {annotated cuboid={width=150, height=200, depth=250, scale=.01, units=m}};
  \pic [fill=gray, text=black, draw=black] at (0,0) {annotated cuboid={width=10, height=10, depth=18, units=}};
  \pic [fill=gray, text=black, draw=black] at (0,-2.0) {annotated cuboid={width=10, height=10, depth=18, units=}};
  \path (0.2, 0.6) node (text1) [texto]{\tiny $Cell_{i-2}$};
  \path (0.2, -3.9) node (text2) [texto]{\tiny $Cell_{i-1}$};
  \path (2.0, -0.28) node (relu) [Phase] {ReLU};
  \path (relu.south)+(0.5, 0) node (conv) [Phase2] {Conv$1\times 1$ };
  \path (conv.south)+(0.5, 0) node (bn) [Phase3] {BN};
  
  \path (2.0, -2.28) node (relu2) [Phase] {ReLU};
  \path (relu2.south)+(0.5, 0) node (conv2) [Phase2] {Conv$1\times 1$ };
  \path (conv2.south)+(0.5, 0) node (bn2) [Phase3] {BN};
  
  \pic [fill=gray, text=black, draw=black] at (5.5,0.2) {annotated cuboid2={width=10, height=10, depth=5, units=}};
  \pic [fill=gray, text=black, draw=black] at (5.5,-1.8) {annotated cuboid2={width=10, height=10, depth=5, units=}};
  
%   \path (bn.south)+(5.0, 1.0) node (celli) [Cell] {\tiny $Cell_i$};
  
  \node[inner sep=0pt, thick, draw] (celli) at (8.7,-1.2){\includegraphics[width=.30\textwidth]{images/DARTS_normal.png}};
  \path (8.7, -0.25) node (text3) [texto]{\tiny $Cell_{i}$};
  
%   \path (phase3)+(3.0, 0.0) node (phase4) [Phase] {Select Init. Ch. and Depth Given ReLU Budget};
  
  \path [draw, ->, line width = 0.3mm] (0.3,-0.28) to (relu.north);
  \path [draw, ->, line width = 0.3mm] (relu.south) to (conv.north);
  \path [draw, ->, line width = 0.3mm] (conv.south) to (bn.north);
  \path [draw, ->, line width = 0.3mm] (bn.south) to (4.5, -0.27);
  
  \path [draw, ->, line width = 0.3mm] (0.3,-2.28) to (relu2.north);
  \path [draw, ->, line width = 0.3mm] (relu2.south) to (conv2.north);
  \path [draw, ->, line width = 0.3mm] (conv2.south) to (bn2.north);
  \path [draw, ->, line width = 0.3mm] (bn2.south) to (4.5, -2.27);
  
  \path [draw, ->, line width = 0.3mm] (5.7, -0.3) to [out=0, in=180] (6.7, -0.6);
  \path [draw, ->, line width = 0.3mm] (5.7, -2.3) to [out=0, in=180] (6.7, -1.6);
  
  \preproc{relu}{relu}{bn2}{bn2}{blue}{Channel Reduction};
  
\end{tikzpicture}
}





% \tikzstyle{Phase}=[draw, fill=gray!10, text width=6.0em, thick, 
%     text centered, minimum width=6.0em, minimum height=3.0em]
% \tikzstyle{texto} = [above, text width=20em, text centered]
% \tikzstyle{Phase2}=[draw, fill=white!10, text width=3.0em, 
%     text centered, minimum width=7.0em, minimum height=4.0em]
% \tikzstyle{Phase3}=[draw, fill=white!10, text width=3.0em, 
%     text centered, minimum width=7.0em, minimum height=4.0em]
% \tikzstyle{CSNode}=[draw, fill=white!10, text width=4.0em, 
%     text centered, minimum width=2.0em, minimum height=6.0em]
% \tikzstyle{restrictionNode}=[draw, fill=white!10, text width=5.0em, 
%     text centered, minimum width=2.0em, minimum height=1.0em]
    
% \newcommand{\phasea}[6]{%
%   \begin{pgfonlayer}{background}
%     % Left-top corner of the background rectangle
%     \path (#1.west |- #2.north)+(-0.3, 0.6) node (a1) {};
%     % Right-bottom corner of the background rectanle
%     \path (#3.east |- #4.south)+(+0.3,-0.6) node (a2) {};
%     % Draw the background
%     \path[fill=#5!20,rounded corners, draw=black!50, dashed]
%       (a1) rectangle (a2);
%     \path (a1.west |- a1.north)+(2.1, -0.65) node (u1)[texto]
%       {\small #6};
%   \end{pgfonlayer}}
  
% \newcommand{\phaseb}[6]{%
%   \begin{pgfonlayer}{background}
%     % Left-top corner of the background rectangle
%     \path (#1.west |- #2.north)+(-0.3, 0.6) node (a1) {};
%     % Right-bottom corner of the background rectanle
%     \path (#3.east |- #4.south)+(+1.6,-0.6) node (a2) {};
%     % Draw the background
%     \path[fill=#5!20,rounded corners, draw=black!50, dashed]
%       (a1) rectangle (a2);
%     \path (a1.west |- a1.north)+(3.1, -0.65) node (u1)[texto]
%       {\small #6};
%   \end{pgfonlayer}}

% \resizebox{1.0\linewidth}{!}{
% \begin{tikzpicture}[font=\sffamily]
%     \fontfamily{cmss}
%     \tikzstyle{every node}=[font=\scriptsize]
    
    
%     \node (phase1) [Phase] {ReLU-Efficient Search Space};
    
%     \path (phase1)+(3.0, 0.0) node (phase2) [Phase] {Candidate Cells \\ from NAS Alg.};
    
%     \path (phase2)+(3.0,0.0) node (phase3) [Phase] {Select Opt. Location of Reduce Cell};
    
%     \path (phase3)+(3.0, 0.0) node (phase4) [Phase] {Select Init. Ch. and Depth Given ReLU Budget};
    
%     \path [draw, ->, line width = 0.3mm] (phase1.east) to (phase2.west);
%     \path [draw, ->, line width = 0.3mm] (phase2.east) to (phase3.west);
%     \path [draw, ->, line width = 0.3mm] (phase3.east) to (phase4.west);
%     \path [draw, ->, line width = 0.3mm] (phase4.east) to node[text width=3.5em, midway, above, align=center]{Performance Evaluation} (11.7, 0);
    
%     \phasea{phase1}{phase1}{phase2}{phase2}{blue}{Stage 1: Finding Cells}
%     \phaseb{phase3}{phase3}{phase4}{phase4}{orange}{Stage 2: Optimizing a Final Skeleton}
    
%     % \path (phase2)+(2.0, 0.0) node (phase3) [Phase1] {Select Opt. Loc. of Reduce Cell};

%     % \path (phase1)+(4.0, 0.0) node (phase3) [Phase3] {Select Opt. Loc. of Reduce Cell};
    
    
    
%     % \path (phase1)+(2.3, 1.5) node (sample) [sampleNode] {\tiny Run Existing NAS Algorithm};
%     % \path (oneShot)+(4, 0) node (CS) [CSNode] {Find optimized reduce cell location via Gumbel-Softmax Trick};
%     % \path (oneShot)+(2.3, -1.6) node (restriction) [restrictionNode] {\tiny Restrict $f$ with \emph{minimizer} of $g$};
    
%     % \path [draw, ->, line width = 0.2mm] (oneShot.north) to (0, 1.5) to (sample.west); 
%     % \path [draw, ->, line width = 0.2mm] (sample.east) to (4, 1.5) to (CS.north);
%     % \path [draw, ->, line width = 0.2mm] (CS.south) to (4, -1.6) to (restriction.east);
%     % \path [draw, ->, line width = 0.2mm] (restriction.north) to (sample.south);
%     % \backgroundc{oneShot}{oneShot}{oneShot}{oneShot}{orange}{Stage 1};
%     % \backgroundd{sample}{sample}{CS}{restriction}{green}{Stage 2};

% \end{tikzpicture}
% }

==> tikz/reduce_cell.tex <==
\tikzstyle{Cell}=[draw, fill=gray!10, text width=4.0em, thick, rounded corners=0.3cm,
    text centered, minimum width=4.0em, minimum height=3.0em]
\tikzstyle{SubCell} = [draw, fill=white!10, text width=2.2em, thick, rounded corners=0.2cm,
    text centered, minimum width=3em, minimum height=2.0em]
\tikzstyle{Cell2}=[draw, fill=gray!10, text width=5.0em, thick, rounded corners=0.2cm,
    align=right, minimum width=6.0em, minimum height=3.0em]
\tikzstyle{texto} = [above, text width=20em, text centered]
\tikzstyle{Image}=[draw, fill=gray!10, text width=3.0em, 
    text centered, minimum width=7.0em, minimum height=4.0em
\tikzstyle{Cell3} = [draw, fill=gray!10, text width=5.0em, thick, rounded corners=0.2cm,
    text centered, minimum width=4.0em, minimum height=3.0em]

\tikzstyle{customNode}=[draw, fill=purple!25, text width=1.0em, 
    text centered, minimum width=1.0em, minimum height=1.0em, rounded corners]
\tikzstyle{customNode2}=[draw, fill=green!25, text width=1.0em, 
    text centered, minimum width=1.0em, minimum height=1.0em, rounded corners]
\tikzstyle{operation}=[draw, fill=white!20, text width=2.0em, 
    text centered, minimum width=2.0em, minimum height=1.0em, rounded corners]
    
\resizebox{0.9\linewidth}{!}{
\begin{tikzpicture}[font=\sffamily, trim left={(0.05,0)}, trim right={(2.8,0)}]
    \fontfamily{cmss}
    \tikzstyle{every node}=[font=\scriptsize]
    
    \node (node0) [customNode] {N0};
    \path (node0)+(0.8, 0.6) node (node1) [customNode] {N1};
    \path (node0)+(1.6, 0) node (node2) [customNode] {N2};
    \path (node2)+(1.2, 0) node (node3) [customNode2] {N3};
    
    \path [draw=brown!80, ->, >=stealth, line width=0.18em] (node0.north) to [out=90, in=180] (node1.west);
    \path [draw=red, ->, >=stealth, line width=0.18em] (node1.east) to [out=0, in=90] (node2.north);
    \path [draw=blue, ->, >=stealth, line width=0.18em] (node0.east) to [out=0, in=180] (node2.west);
    \path [draw=black, ->, >=stealth, line width=0.18em] (node2.east) to [out=0, in=180] (node3.west);
    \path [draw=black, ->, >=stealth, line width=0.18em] (node0.south) to [out=320, in=180] (1.4, -0.6) to [out=0, in=220] (node3.south);
    \path [draw=black, ->, >=stealth, line width=0.18em] (node1.east) to [out=0, in=140] (node3.north);
\end{tikzpicture}
}

==> tikz/summary.tex <==
%\resizebox{\linewidth}{!}{%neurips
\tikzstyle{Phase}=[draw, fill=gray!10, text width=6.0em, thick, 
    text centered, minimum width=6.0em, minimum height=3.0em]
\tikzstyle{texto} = [above, text width=20em, text centered]
\tikzstyle{Phase2}=[draw, fill=white!10, text width=3.0em, 
    text centered, minimum width=7.0em, minimum height=4.0em]
\tikzstyle{Phase3}=[draw, fill=white!10, text width=3.0em, 
    text centered, minimum width=7.0em, minimum height=4.0em]
\tikzstyle{CSNode}=[draw, fill=white!10, text width=4.0em, 
    text centered, minimum width=2.0em, minimum height=6.0em]
\tikzstyle{restrictionNode}=[draw, fill=white!10, text width=5.0em, 
    text centered, minimum width=2.0em, minimum height=1.0em]
    
\newcommand{\phasea}[6]{%
  \begin{pgfonlayer}{background}
    % Left-top corner of the background rectangle
    \path (#1.west |- #2.north)+(-0.3, 0.6) node (a1) {};
    % Right-bottom corner of the background rectanle
    \path (#3.east |- #4.south)+(+0.3,-0.6) node (a2) {};
    % Draw the background
    \path[fill=#5!20,rounded corners, draw=black!50, dashed]
      (a1) rectangle (a2);
    \path (a1.west |- a1.north)+(2.1, -0.65) node (u1)[texto]
      {\small #6};
  \end{pgfonlayer}}
  
\newcommand{\phaseb}[6]{%
  \begin{pgfonlayer}{background}
    % Left-top corner of the background rectangle
    \path (#1.west |- #2.north)+(-0.3, 0.6) node (a1) {};
    % Right-bottom corner of the background rectanle
    \path (#3.east |- #4.south)+(+1.6,-0.6) node (a2) {};
    % Draw the background
    \path[fill=#5!20,rounded corners, draw=black!50, dashed]
      (a1) rectangle (a2);
    \path (a1.west |- a1.north)+(3.1, -0.65) node (u1)[texto]
      {\small #6};
  \end{pgfonlayer}}

\resizebox{1.0\linewidth}{!}{
\begin{tikzpicture}[font=\sffamily, trim left={(-1.5,0.0)}]
    \fontfamily{cmss}
    \tikzstyle{every node}=[font=\scriptsize]
    
    
    \node (phase1) [Phase] {ReLU-Efficient Search Space};
    
    \path (phase1)+(3.0, 0.0) node (phase2) [Phase] {Candidate Cells \\ from NAS Alg.};
    
    \path (phase2)+(3.0,0.0) node (phase3) [Phase] {Select Init. Ch. and Depth Given ReLU Budget};
    
    \path (phase3)+(3.0, 0.0) node (phase4) [Phase] {Search Optimal Location of Reduce Cell};
    
    \path [draw, ->, line width = 0.3mm] (phase1.east) to (phase2.west);
    \path [draw, ->, line width = 0.3mm] (phase2.east) to (phase3.west);
    \path [draw, ->, line width = 0.3mm] (phase3.east) to (phase4.west);
    \path [draw, ->, line width = 0.3mm] (phase4.east) to node[text width=3.5em, midway, above, align=center]{Performance Evaluation} (11.7, 0);
    
    \phasea{phase1}{phase1}{phase2}{phase2}{blue}{Stage 1: Finding Cells}
    \phaseb{phase3}{phase3}{phase4}{phase4}{orange}{Stage 2: Optimizing a Final Skeleton}
    
    % \path (phase2)+(2.0, 0.0) node (phase3) [Phase1] {Select Opt. Loc. of Reduce Cell};

    % \path (phase1)+(4.0, 0.0) node (phase3) [Phase3] {Select Opt. Loc. of Reduce Cell};
    
    
    
    % \path (phase1)+(2.3, 1.5) node (sample) [sampleNode] {\tiny Run Existing NAS Algorithm};
    % \path (oneShot)+(4, 0) node (CS) [CSNode] {Find optimized reduce cell location via Gumbel-Softmax Trick};
    % \path (oneShot)+(2.3, -1.6) node (restriction) [restrictionNode] {\tiny Restrict $f$ with \emph{minimizer} of $g$};
    
    % \path [draw, ->, line width = 0.2mm] (oneShot.north) to (0, 1.5) to (sample.west); 
    % \path [draw, ->, line width = 0.2mm] (sample.east) to (4, 1.5) to (CS.north);
    % \path [draw, ->, line width = 0.2mm] (CS.south) to (4, -1.6) to (restriction.east);
    % \path [draw, ->, line width = 0.2mm] (restriction.north) to (sample.south);
    % \backgroundc{oneShot}{oneShot}{oneShot}{oneShot}{orange}{Stage 1};
    % \backgroundd{sample}{sample}{CS}{restriction}{green}{Stage 2};

\end{tikzpicture}
}
